SS-SFDA : Self-Supervised Source-Free Domain Adaptation for Road Segmentation in Hazardous Environments

We present a novel approach for unsupervised road segmentation in adverse weather conditions such as rain or fog. This includes a new algorithm for source-free domain adaptation (SFDA) using self-supervised learning. Moreover, our approach uses several techniques to address various challenges in SFDA and improve performance, including online generation of pseudo-labels and self-attention as well as use of curriculum learning, entropy minimization and model distillation. We have evaluated the performance on $6$ datasets corresponding to real and synthetic adverse weather conditions. Our method outperforms all prior works on unsupervised road segmentation and SFDA by at least 10.26%, and improves the training time by 18-180x. Moreover, our self-supervised algorithm exhibits similar accuracy performance in terms of mIOU score as compared to prior supervised methods.

==> Tables/AblationsSOTA/suppWeather.tex <==
\begin{table}[H]
% \footnotesize
\label{tab:supp_datasets}
\centering
% \begin{center}
 \resizebox{\textwidth}{!}{
%\resizebox{\columnwidth}{!}{
\begin{tabular}{r c c c c}
\toprule
Dataset & Syn./Real & Weather & Time of Day & Image Size\\
\midrule
Rainy CityScapes \cite{halder2019physics}& Syn & Varying intensities (1mm - 200mm) of rain & Daytime & $512,1024$\\
Foggy CityScapes \cite{halder2019physics}& Syn & Varying intensities (750m - 30m) of fog & Daytime & $512,1024$\\
Foggy Zurich \cite{sakaridis2018model}& Real & Light and medium Fog & Daytime & $540,960$\\
Dark Zurich \cite{sakaridis2019guided}& Real & Clear & Twilight, Night &  $540,960$\\
Raincouver \cite{tung2017raincouver}& Real & Rain & Twilight, Night & $360,640$ \\
BDD \cite{yu2018bdd100k}& Real & Clear, Snow, Fog, Rain & Daytime, Twilight, Night & $720,1280$\\

\bottomrule
\end{tabular}

} %For resize box
% \caption{\textbf{List of datasets:} The second column categorizes the datasets as synthetic or real and the third, fourth and fifth columns describe the images contained in the dataset.}
% \vspace{-15pt}
% \end{center}
\end{table}




==> Tables/Supervised/ablations_clearcityscapes.tex <==
\begin{table}
% \footnotesize
\centering
% \begin{center}
% \resizebox{.8\columnwidth}{!}{
\begin{tabular}{c c c c c}
\toprule
Model & mIoU & Recall & Prec. & F1 \\
\midrule
\multicolumn{5}{c}{I. Ablations on the loss formulations on DeepLabv2(Enc-2)}\\
\midrule
MSE Loss & $88.77$&	$94.86$&	$93.25$&	$94.05$\\
L1 loss & $88.69$	& $94.48$&	$93.53$&	$94.00$\\
BCE Loss & $88.62$&	$94.54$&	$93.39$&	$93.96$\\
\midrule
\multicolumn{5}{c}{II. Ablations on the evaluation probability} \\ \multicolumn{5}{c}{threshold $\tau$ on DeepLabv2(Enc-2)}\\
\midrule
$0.4$ & $88.63$	& $95.65$	& $92.34$	& $93.97$ \\
$0.5$ & $88.62$ &	$94.54$ & 	$93.39$ &	$93.96$\\
$0.6$ & $88.29$	& $93.23$ &	$94.33$	& $93.78$\\
\bottomrule
\end{tabular}
% }
\caption{Clear weather cityscapes ablations}
\label{tab:cityscapesclearweather_ablations}
\vspace{-12pts}

% \end{center}
\end{table}




==> Tables/WeatherDatasets/syntheticfog.tex <==
\begin{table}
% \footnotesize
\centering
% \begin{center}
\resizebox{.8\columnwidth}{!}{
\begin{tabular}{c c c c c c}
\toprule
Visibility & Experiment & mIoU & Recall & Prec. & F1 \\
\midrule
%\midrule
%\multicolumn{5}{c}{Light Fog, Experiment A}\\
750 m & A & 94.90	& 96.68&	98.09&	97.38\\
375 m & A & 92.71 &	94.60&	97.88&	96.21\\
\midrule
%\midrule
%\multicolumn{5}{c}{Fog 150m}\\
150m & A & 85.55&	87.57&	97.38&	92.21\\
150m & B & 89.74&	94.59&	94.59&	94.59\\
%\midrule
\midrule
%\multicolumn{5}{c}{Fog 75m}\\
75m & A & 70.81 &	72.51 &	96.79 &	82.9\\
75m & B & 80.67 &	83.01 &	96.62 &	89.30\\
75m & C & 87.48&	92.99&	93.65&	93.32\\
%\midrule
\midrule
%\multicolumn{5}{c}{Fog 50m}\\
50m & A & 57.29 &	58.92&	95.39&	72.85\\
50m & B & 71.64&	73.69&	96.24&	83.47\\
50m & C & 85.47&	90.75&	93.63&	92.16\\
\midrule
%\midrule
%\multicolumn{5}{c}{Fog 40m}\\
40m & A & 46.27&	48.45&	91.12&	63.27\\
40m & B & 52.62 &	53.94&	95.57&	68.96\\
40m & C & 83.65 &	89.19&	93.09&	91.10\\
%\midrule
\midrule
%\multicolumn{5}{c}{Fog 30m}\\
30m & A & 35.04&	38.05&	81.59&	51.90\\
30m & B & 22.24&	22.92&	88.29&	36.39\\
30m & C & 80.82 &	85.96&	93.11&	89.39\\
%\midrule


\bottomrule
\end{tabular}
}
\caption{\textbf{Results on synthetic fog:} We evaluate the model under three settings - A: Testing the clear weather CityScapes model, B: \model~ without curriculum learning, C: \model~. We show that he CityScapes model generalizes well to light synthetic fog, and its performance degrades severely as the intensity of fog increases, which is restored by \model~. \model~ achieves 90.8\%-96.78\% and 91.12\%-98.82\% of supervised mIoU and recall, respectively. }
\label{tab:syntheticfog_mainresults}
\vspace{-12pt}

% \end{center}
\end{table}



